A survey of algorithmic recourse: definitions, formulations, solutions, and prospects

Machine learning is increasingly used to inform decision-making in sensitive situations where decisions have consequential effects on individuals' lives. In these settings, in addition to requiring models to be accurate and robust, socially relevant values such as fairness, privacy, accountability, and explainability play an important role for the adoption and impact of said technologies. In this work, we focus on algorithmic recourse, which is concerned with providing explanations and recommendations to individuals who are unfavourably treated by automated decision-making systems. We first perform an extensive literature review, and align the efforts of many authors by presenting unified definitions, formulations, and solutions to recourse. Then, we provide an overview of the prospective research directions towards which the community may engage, challenging existing assumptions and making explicit connections to other ethical challenges such as security, privacy, and fairness.

==> 050discussion.tex <==
% \amir{TODO: clean up this section; currently just a brain dump}

% \bernhard{will edit here next}

==> 051promise.tex <==
% \subsection{Promise}

In \S\ref{sec:020background}, we showed that generating recourse explanations and recommendations required counterfactual reasoning at various levels of the causal history.
%
Counterfactual reasoning has roots not only in the philosophy of science \citep{lipton1990contrastive, hilton1986knowledge, hilton1990conversational, lewis1973counterfactuals, lewis1986causal, woodward2005making}, but also in the psychology of human agents \citep{miller2018contrastive, miller2019explanation, byrne2019counterfactuals}, and benefits from strong technical foundations \citep{halpern2005causes, bareinboim2020pearl}.
%
User studies have demonstrated that causal relationships are assessed by evaluating counterfactuals \citep{mcgill1993contrastive}, and counterfactual simulation is used to predict future events \citep{gerstenberg2017eye}.
%
Specifically in the context of XAI, it has been shown that counterfactuals can ``make the decisions of inscrutable systems intelligible to developers and users'' \citep{byrne2019counterfactuals}, and that people perform better at predicting model behavior when presented with counterfactual instances \citep{lage2019evaluation}.
%
Organizations seek to deploy counterfactual-based explanations citing their easy-to-understand nature \citep{bhatt2020explainable, bhatt2020machine} and GDPR-compliance \citep{wachter2017counterfactual}.
%
Finally, from a practitioner's standpoint, not only does algorithmic recourse benefit from the widely exercised practice of sharing open-source implementations (see Table~\ref{table:technical_summary}), various graphical interfaces have also been developed to assist the on-boarding of non-technical stakeholders \citep{wexler2019if, cheng2020dece, gomez2020vice}.


% ideas:
% \begin{itemize}
%     \item some user studies that should this recourse is useful?
%     \item see backup file;
%     \item perhaps cite umang's work;
%     \item perhaps read dece paper
%     \item page 3 of \url{https://arxiv.org/pdf/2005.13997.pdf}
%     \item \url{http://interactions.acm.org/archive/view/july-august-2019/10-things-you-should-know-about-algorithmic-fairness}
% \end{itemize}

% While explainability and interpretability have significant potential upside, there are a lot of open questions regarding their viability. The extent to which explainability and interpretability are achievable, particularly with existing machine learning technologies, is a matter of open debate. Further, they may come with costs; for example, systems that are more understandable may be more vulnerable to manipulation and hacking. However, in the algorithmic fairness space, explainability and interpretability largely appear to be a means to an end rather than an end goal, and alternative properties may be more useful. In my experience, stakeholders asking for explainability and interpretability in the pursuit of algorithmic fairness are actually often seeking related properties that have recently been articulated in FAT* and related communities, such as contestability [8] (the ability to challenge decisions made by machine learning systems) or recourse [9] (the ability to change the decision of the model via actionable changes to input variables). There is an emergent understanding that different properties meet different needs. For example, a plaintiff in a lawsuit may need something very different from a doctor using a system to inform a medical diagnosis. However, there is not yet a clear understanding of which properties are needed by which stakeholders at which times and for which purposes, and user research elucidating these needs would greatly advance the field.


% \subsubsection{\textbf{historical shaping of algorithmic phenomena; algorithmic impacts on social phenomena}}
% \hl{from FAccT CFP} \url{https://facctconference.org/2021/cfp.html}
% \amir{bias in dataset even more (see into equalizing recourse across groups)}












% \subsubsection{\textbf{More from Barocas and Venkatasubramanian?}}

% \subsubsection{\textbf{Interventionist interpretation of recourse}}
% \url{https://plato.stanford.edu/entries/causation-mani/#InteCoun}

==> 052problems.tex <==
\subsection{Problems}

Here, we present two technical areas where recourse could be improved, complementing the critiques in \cite{venkatasubramanianphilosophical, barocas2020hidden}.

\subsubsection{\textbf{On the lack of benchmarks}}
% Earlier, we presented the general recourse formulations, for both contrastive explanations and consequential recommendations, and reviewed the variety of objectives and constraints employed to model real-world settings (see also Table \ref{table:technical_summary}). %and mentioned that it is NP-hard both in general and in simplified settings.
%
% Table \ref{table:technical_summary} summarized papers that offer recourse in a variety of settings, which are supported by robust tools and perform well.
%
Table \ref{table:technical_summary} presented an overview of the diverse settings in which recourse is sought.
%
Despite the abundance of open-source implementations built on robust tools and working well in their respective settings, a comparative benchmark for recourse is lacking.
%
This problem is exacerbated for consequential recommendations which further rely on assumptions about the causal generative process. % missing due to identifiability issues \hl{cite}.
%
In order to make objective progress, however, new contributions should be evaluated against existing methods. 
%
Thus, a next step for the community is the curation of an online challenge (e.g., using Kaggle) to benchmark the performance of existing and new methods.
%
To broadly cover practical settings, we envision multiple tracks where authors can submit their generated explanations/recommendations given a fixed classifier, test dataset, and pre-determined \dist/\cost\, definition, and be evaluated using the metrics defined in \S\ref{sec:solutions_properties}.
%
Authors may also submit results that satisfy additional actionability, plausibility, and diversity constraints, and be compared as such.

% %
% As a result, most papers evaluate their method in specific settings, e.g., on real-valued datasets, assuming differentiable models and objective, or under white-box access to the model. 
% %
% Thus, it is easy to understand why, despite most papers having accompanying open-source implementations, a comparative benchmark is lacking.
% %
% This problem is exacerbated for consequential recommendations which further rely on specification of the causal generative process missing due to identifiability issues \hl{cite}.
% %
% % Finally, due to variety of desirable metrics in these approximate settings, one can expect that algorithmic choices are made such that the resulting solution falls on a Pareto front of competing objectives.
% % Finally, due to the multi-objective setup (with optimality, diversity, etc.), one can expect that algorithmic choices are made such that the resulting solution falls on a Pareto front of competing objectives.
%


% \hl{papers with code / kaggle}
% lack of benchmarks (formulations, datasets, and universal metrics), DUE TO user-/context-specific objective/cost, feasibility, etc. and difficulty of optimization


% \subsubsection{\textbf{On the cost of recourse}}
\subsubsection{\textbf{On the definition of \dist\, and \cost}}
\label{sec:cost_of_recourse}

% Although objective definitions of dissimilarity between individuals and cost of actions have been elusive in both the fairness and recourse literature (see \S\ref{sec:objective}), \hl{we consider the following properties as primitives:} % a potential guideline:

% % To capture the preference for minimal \cost\, actions, or for small \dist\, between factual and counterfactual instances, early works suggest the following properties: %we follow \cite{ustun2019actionable} and suggest the following axioms:
% %existing approaches posit that distance/cost functions should satisfy the following properties:
% \begin{itemize}
%     \item[\textbf{P1:}] no action $\Leftrightarrow$ no cost $\Leftrightarrow$ no distance
%         \newline i.e., $\cost(\zvec{0}; \xF) = 0 = \dist(\xF, \xF)$ % for $\xCF = \xF + \thetaVector$,
%         % \newline or $\cost(\mathbbm{1}; \xF) = 0 = \dist(\xF, \xF)$ for $\xCFnearest = \actionVectorStar \cdot \xF$
%     \item[\textbf{P2:}] larger actions $\Leftrightarrow$ higher cost $\not\Leftrightarrow$ larger distance
%         \newline i.e., $\cost(\actionVector; \xF) \le \cost(\actionVector + \epsilon \mathbbm{1}_j ; \xF)$
%         \newline i.e., \hbox{$\theta_1 \le \theta_2 \implies \cost(\doop(\xF_i + \theta_1); \xF) \le \cost(\doop(\xF_i + \theta_2); \xF)$}
% \end{itemize}

% % We highlight a subtlety in \textbf{P1}: although the cost of no action on all features is 0, the cost of holding a variable at

Definitions of dissimilarity between individuals and cost of actions have been elusive in both the fairness and recourse literature. % (see \S\ref{sec:objective}).
%
In \S\ref{sec:objective}, we suggested that in a world in which changing one variable does not affect others, \dist\, and \cost\, \emph{may} be used interchangeably, which breaks down when variables are causally dependent.
%
In general, however, we do not consider a \hbox{1-1} mapping between effort expended by an individual (i.e., \cost) and dissimilarity between individuals (i.e., \dist). % , as in \textbf{P2} 
%
For instance, in a two-variable system with \variable{medication} as the parent of \variable{headache}, an individual that consumes more than the recommended amount of medication may not recover from the headache, i.e., higher cost but smaller \emph{symptomatic} distance relative to another individual who consumed the correct amount.
%
Furthermore, while dissimilarity is often considered to be symmetric (i.e., $\dist(\xF_A, \xF_B) = \dist(\xF_B, \xF_A)$), the effort needed to go from one profile to another need not satisfy symmetry, e.g., spending money is easier than saving money (i.e., $\cost(\actionVector = \doop(\zrv{X}_{\$} := \xF_{A,\$} - \$500); \xF_A) \le \cost(\actionVector = \doop(\zrv{X}_{\$} := \xF_{B,\$} + \$500); \xF_B)$.
%
These example illustrate that the interdisciplinary community must continue to engage to define the distinct notions of \dist\, and \cost, and such definitions cannot arise from a technical perspective alone.







% While \textbf{P1} holds in both independent and dependent worlds, \textbf{P2} may not hold in dependent worlds where intervening on one variable may positively/negatively affect other variables.
% %
% For instance, in a two-variable system with \variable{medication} as the parent of \variable{headache}, an individual that consumes more than the recommended amount of medication may end up with a stronger headache, i.e., higher cost but perhaps smaller distance relative to another individual who consumed the correct amount.
% %
% \amirr{causality matters}
% A natural way to address this shortcoming is to distinguish between \emph{cost of actions} and \emph{cost of consequences of actions}, equating the latter to the cost of non-altering interventions on descendants of the intervened-upon variables.
% %
% This assignment holds intuitively: when consequences of actions are beneficial (resp. detrimental) towards the output of $\htheta$, the latter cost captures the opportunity cost (resp. preventative cost) of non-altering interventions.
% %
% Although objective definitions of dissimilarity of individuals and cost of actions have been elusive in both the fairness and recourse literature (see \S\ref{sec:objective}), such a distinction may prove useful towards a set of axioms for the cost of recourse.
% % \hl{Finally, recent work attempts to learn dissimilarity from the data itself; AReS Bradley-Terry}.

%
% While \textbf{P1} holds in both independent and dependent worlds, \textbf{P2} fails in dependent worlds where the cost of non-altering interventions -- necessary to ensure that $\xSCF$ equals $\xCFnearest$ -- is overlooked.
% %
% \hl{For instance, the agriculture team in Example \#2 of} \S\ref{sec:010introduction} \hl{may need to invest heavily in a greenhouse to ensure temperature remains the same if the paddy were to be situated at a different altitude.}
% %
% A natural way to address this shortcoming is to distinguish between \emph{cost of actions} and \emph{cost of consequences of actions}, \hbox{equating the latter to the} cost of non-altering interventions.
% %
% This assignment holds intuitively: when consequences of actions are beneficial (resp. detrimental) towards the output of $\htheta$, \hbox{the latter cost captures} the opportunity cost (resp. preventative cost) of non-altering interventions.

% The implementation of the proposed two-part cost function, however, involves a functional of not only $\actionVector$ and $\xF$, but also of $\scmModel$ and $\htheta$.
% %
% Furthermore, notions of cost and distance are notoriously difficult to define and not universally agreed upon \citep{dwork2012fairness, ilvento2019metric, venkatasubramanianphilosophical}.
% %
% In the spirit of not complicating matters further, we adopt the existing properties of cost functions (i.e., \textbf{P1}, \textbf{P2}), and propose a modification of \hl{eqn:nearest-cf-additive} that allows for \hl{actionSetStar} to \emph{optimally} and \emph{feasibly} follow via Option \#1, thereby avoiding the concerns of non-altering interventions.
% %
% % We present our approach in the following section, and defer the exploration of alternative cost definitions to future work.
% \hl{talk also about cost of actions performed by fiduciary or background variables}.
% %




==> 059recourseprivacy.tex <==
\amirm{privacy violation}
Building on the intuition of the previous section, we note that explanations may indirectly expose the predictions of similar individuals.
%
In more detail, a contrastive explanation informs the data-subject that there are no instances in a certain vicinity (i.e., within $\ballF$) such that their prediction is different (otherwise that would be the nearest contrastive explanation).
%
This information informs the data-subject about, e.g., whether their similar friend was also denied a loan, violating their predictive privacy.
%
Even under partial knowledge of the friend's attributes, an adversary can use the information about the shared predictions in $\ballF$ to perform membership inference attacks \citep{shokri2019privacy} or infer missing attributes \citep{dwork2018privacy}.
%
This problem is worsened when multiple diverse explanations are generated, and is an open problem.


==> _bu_020background.tex <==



% Different definitions of CFE:
% \begin{itemize}
%   \item contrastive explanations in \citep{dhurandhar2018explanations}
%   \item counterfactual
%   \item SEDC in \citep{vermeire2020explainable}
%   \item Provost in \citep{fernandez2020explaining}
% \end{itemize}






% Ustun:

% In the relatively nascent field of algorithmic recourse, recourse is defined as ``the ability of a person to obtain a desired outcome from a fixed model''.

% Seeing how the lack of autonomy is perceived as a source of injustice in algorithmic decision-making [6, 14, 33],

% The study of recourse involves determining the existence and di culty of actions to obtain a desired prediction from a  xed machine learning model. Such actions do not re ect the principle reasons for the prediction (c.f., explainability), and are not designed to reveal the operational process of the model (c.f., transparency).



% Joshi:
% Individual recourse pertains to the problem of providing an actionable set of changes a person can undertake in order to improve their outcome



% Gupta:

% recourse for negative decisions should be considered a desirable value that can be equalized across

% We measure recourse as the distance of an individual from the decision boundary of a classifier

% One way in which we have traditionally placed checks on the power of decision-making systems, especially in settings where the decisions may have significant effects on our lives, is by providing the subject of the decision with a mechanism for recourse [USL19]: the ability to ask how the decision was made and what can be done to change it.

% This idea of recourse is a part of the Equal Credit Opportunity Act –an individual can demand that reasons for a loan denial be provided – and research suggests that it might also eventually be a component of the right to explanation implicated in the General Data Protection Regulation of the European Union

% But the idea of recourse is more than a legal concept: it can be viewed as an ethical and just way to make decision-making more transparent. If a decision that materially affects us is made using factors that we cannot realistically change (for example a decision based on our gender or race), then this decision eliminates our agency and is therefore unjust [RCP]. Thus providing opportunities for recourse is a valuable goal independent of concerns about fairness and non-discrimination.



% Suresh:

% recourse – the systematic process of reversing unfavorable decisions by algorithms and bureaucracies across a range of counterfactual scenarios – is such a modally ro- bust good. In particular, we argue that two essential components of a good life – temporally extended agency and trust – are under- written by recourse.

% As such, we need some way to ensure that people both have some way of getting unfavorable decisions reversed and know, in general, that they will have a way of getting unfavorable decisions reversed. Let us de ne the enjoyment of recourse as being in such a position. Recourse systematically delivers the bene t of reversing harmful decisions by algorithms and bureaucracies across a range of counterfactual scenarios4. If someone enjoys recourse, then not only are they able to get a single decision reversed, but they also enjoy the power to reverse decisions across a range of counterfac- tual scenarios. As such, someone who enjoys recourse need not passively su er the slings and arrows of outrageous fortune, but is positioned to take up arms against a sea of troubles

% Thus, we distinguish between particular token acts of exercising recourse (reversing a single harmful decision) and the general state of enjoying systematic access to the power to reverse harmful decisions (knowing that if a harmful decision were to be made, one would be able to get it reversed).

% For Kant (e.g., Groundwork 4:431) and his interpreters (e.g., [35], [20], [15]), dignity is grounded in humanity, which in turn is typ- ically understood as involving two closely-connected capacities. First, humanity involves the capacity to select ends or goals. Sec- ond, humanity involves the capacity to be autonomous. It should be clear from the discussion in the previous section that the ca- pacity to select goals is deeply dependent on the sort of long-term, temporally-extended agency that recourse makes possible. What about autonomy? While there are of course disagreements among interpreters about how best to understand Kantian autonomy, ac- cording to the Stanford Encyclopedia of Philosophy, it involves "the capacity to freely direct, shape, and determine the meaning of one’s own life" [7]. Again, this seems to be exactly the sort of long-term planning and self-direction that recourse as we have formulated it helps to secure.

% Other philosophers working in the deontological tradition with- out hewing quite as closely to the orthodox Kantian line o er similar analyses of the meaning and importance of dignity. For example, Gri n [12] contends that the source of human dignity is our ca- pacity to form, revise, and pursue what we take to be worthwhile lives. Likewise, Raz [28] says that "Respecting human dignity en- tails treating humans as persons capable of planning and plotting their future." And Fuller [10] emphasizes that constraints on human agency thus understood should be understandable to the people on whom they are imposed. One very clear way in which to make the constraints under which someone operates understandable to them is to explain what it would take for the rules (including algorithmic rules) to spit out a di erent result.

% These re ections suggest that – regardless of whether you favor a consequentialist or a deontological normative ethical framework – recourse will turn out to be a fundamental good for anyone who lives in the sort of society that many people currently inhabit. Unless we think that algorithmic and bureaucratic systems – which exist in domains as diverse as criminal justice, credit scoring, hiring, insurance, and voter certi cation – are or could soon be made infallible, we must place a high value on recourse, on the ability to know what it would take to get a di erent outcome from high- stakes decisions arrived at by algorithms and bureaucracies.

% Recourse is quanti ed as a “distance from the decision boundary.”

% Work on recourse builds on earlier research on explanations in machine learning via counterfactuals by Wachter et al.[32]. In that work, the authors argue that, for a number of reasons linked to considerations provided by the European General Data Protection Regulation (GDPR), it would be bene cial to have counterfactual explanations of decisions. A counterfactual explanation is of the form “If variable V took di erent values, the decision would have been di erent.” 9 Wachter et al. argue that such explanations furnish the information necessary to contest decisions as well as exercise recourse, and they suggest ways in which one might produce such a counterfactual from a given model.

% Counterfactual explanations have proven to be a popular frame- work for generating explanations[18, 29]. However, an explanation in and of itself need not provide recourse if it is merely provid- ing insight into the decision process of the system. In this paper we focus on recourse directly because of its connection to trust and temporally-extended agency, but many of our critiques and interventions can be applied when appropriate to other forms of explanations. For a detailed exposition of the nature of explana- tions in decision-making, see the work of Selbst and Barocas [30]. Barocas, Selbst and Raghavan[4] provide a more focused critique of counterfactual explanations.
























% \newpage
% % \vspace{3cm}
% \subsection{Interpretable Machine Learning}

% \amir{funnel diagram, xai, then model-based and feature-based, then some examples of feature-based (shap, lime, etc.), then counterfactual/contrastive explanations}

% Talk about stakeholders.. then zoom into consequential decision making setting, then focus on data-subjects.

% Consider Figure \hl{1}, depicted the life cycle of a machine learning model. \hl{review/cite papers on stakeholders + Umang}
% %
% In a standard setting, we have a researcher or engineer (\hl{Fig 1a}), who develops a model with certain objective measures based on the information of data-subjects (\hl{Fig 1b}).
% %
% This model is in turn owned and deployed by another individual/institution (\hl{Fig 1c}), which when deployed turns data-subjects into decision subjects.
% %
% All the while, the law or a regulatory body aims to assay that there are no disparities in the process and privacy is handled accordingly (\hl{Fig 1d}).

% Even in this simple schema, intepretability can mean various things to the different stakeholders involved.
% %
% Their needs may even at times be at odds \hl{give examples}



% \subsection{Causal \& Counterfactual Reasoning}

% \amir{discuss: brief of counterfactuals: Lewis + Hume + Pearl}

% Several formal models of causation have been proposed, including \hl{...SEP/Miller...}
% %
% In this work, we adopt the \emph{Structural Causal Model} (SCM) framework of \citet{pearl2000causality}, as it is simpler to understand and manipulate with tools of probability and graph theory, and thus easily accessible to the audience of this work.
% %
% An SCM is comprised of a four-tuple ($\zset{F}, \zset{X}, \zset{U}, P_U$), where... \hl{Elias' paper}







% \subsection{rando}
% Import In this context, in addition to negating causes or effects, additional properties are required of the explanation.
% %
% Specifically, minimum effort



% % To prevent confusion and while they are both broadly classified as counterfactual (in th it is important to distinguish between



% As we shall see below, while many works on recourse present explanations to the first query, answering the second question in real-world settings would involve \hl{causal attribution} and.... \citep{karimi2020mintrecourse}.

% This is because the answer to second query involves actions and effort that the individual must expend to acheive a desired output, and thus.. \

% % To answer the first question, one might consider that the only variables that affect the output of the decision-making system are the inputs. In a sense, we could argue that the input covariates, $\xAny$, are causes for the output prediction, $\hat{y}$.
% % %
% % Thus, in this simple world the relative importance of features may be a sufficient explanation. The relation between features may optionally be considered (as in cite janzing and others etc.) or assumed to be independent (as in cite) when measuring causal attribution relative to the black-box decision-making system.

% However, social science and psychology literature suggest that in seeking the answer to ``why p not q'', human often don't care about the entire causal history (and it's often difficult to automatically learn anyways). Thus, questions of the first type are better answered contrastively and may be reformulated as:

% \begin{enumerate}
%     \item Who should I become in order to receive the loan?
%     \item How should I become the aforementioned profile?
% \end{enumerate}





% % \subsection{Clarifying terminology: \\ contrastive vs. counterfactual}

% % \hl{something something causal explanations, causal attribution}.

% % Consider two variables, $\zrv{X}$ and $\zrv{Y}$, where $\zrv{X}$ is a potential cause of the observed effect, $\zrv{Y}$.
% % %
% % E.g., $\zrv{X}$ is a tuple of \variable{age}, \variable{gender}, and \variable{profession} of an individual loan-seeker, and $\zrv{Y}$ corresponds to their \variable{salary/loan status}.
% % %
% % Consider the 28-year-old female candidate from the previous example, who was denied a loan. To present recourse, the first question we should answer is why was....

% % Recent research falls into two camps when assessing causal explanation/attribution.
% % %
% % The first camp evaluates causal attribution in terms of the counterfactual statement: ``Would $\zrv{Y}$ have occurred if $\zrv{X}$ had not?''

% % The second camp considers the contrastive statement


% % \amir{define the basic constrained optimization formulation, to motivate the table?? or defer to section 3}






































\citet{lipton1990contrastive} posits that the answer to a contrastive questions is a \emph{Difference Condition}, where

To explain why P rather than Q, we must cite a causal difference between P and not-Q, consisting of a cause of P and the absence of a corresponding event in the history of not-Q. – Lipton [19, p. 256].
Following this, the explainer does not need to reason about or even know about all causes of the fact — only those relative to the contrast case.

This seems to align with

The key insight is to recognise that one does not explain events per se, but that one explains why the puzzling event occurred in the target cases but not in some counterfactual contrast case — Hilton [14, p. 67].



don't provide the entire causal history, but only enough to differentiate between p and q: difference condition


Whereas generating contrastive explanations does not depend on knowledge of the causal relations between variables, generating consequential interventions does.
%
In fact, \citet{karimi2020caterecourse} showed that recourse actions cannot be offered if the true SCM is unknown.





the requirements above for explanations and recommendations align well with what is available in our setting, a fixed model, input variables, which for the purpose of contrastive explanation may be considered independent (minimum change in causal past, relative to the fixed model), but for recommendations, cannot be considered as such.

both can be considered as counterfactual as something is negated.

thus the two questions become

\begin{enumerate}
    \item Who should I become in order to receive the loan?
    \item What interventions should I perform to receive the loan?
\end{enumerate}



\subsubsection{\textbf{On the relation between contrastive explanations and consequential interventions}}
need not overlap... see brief text in \S\ref{sec:030formulation}

\begin{figure}[t]
    \caption{To guarantee recourse (i.e., flip the prediction), one must negate a cause in the causal history of the output of the fixed model. Whereas for contrastive explanation it is sufficient to changing the feature vector $x_1 \cdots x_d$, in consequential interventions one must consider negating variable values and consider the consequence of this action on other variables.}
    \centering
    \includegraphics[width=\linewidth]{recourse.jpg}
\end{figure}


A formal and comprehensive review of the definitions, goals, and forms of explanation falls outside the scope of this work; we refer the reader to e

Cite some famous folks
  what types of explanations are considered
    contrastive is important, both philosophically and psychologically and socially
      thus the first question becomes why did i not get the loan (rather than get)
        rewrite two questions

something something diagram

something something why structural counterfactuals are important

As suggested by \citet{mcgill1993contrastive, miller2019explanation}, ``both counterfactual and contrastive reasoning may be broadly classified as counterfactual, in that each considers instances in which some characteristic of the event (cause or effect) has been negated.'' \hl{negated/changed... we want to minimize the change, either in the effect (contrastive explanation) or in the cause (consequential interventions).}


% \clearpage

% \subsection{Philosophy of recourse/explanations: contrastive vs. counterfactual}
% \subsection{Recourse via contrastive and counterfactual explanations}
\subsection{Clarifying terminology: counterfactual, contrastive, and consequential}
% \subsection{Recourse via contrastive explanations\\and consequential interventions}
\zmessage{ we require related but different reasoning.}

We recall the definition of \emph{explanation} from \citet[p. 217]{lewis1986causal} where ``to explain an event is to provide some information about its causal history.''


To generate \hl{causal explanations}, one line of research suggests that \emph{counterfactual reasoning} is used to answer the first question~\citep{einhorn1986judging, wells1989mental, lipe1991counterfactual}.
%
This would involve trying to determine, through mental simulation, whether or not the individual would have been offered the loan had her characteristics been different (e.g., had she been male, or had her salary been higher).
%
% In experimental studies, people have shown to use either mental simulation \hl{cite} or existing covariate information \hl{cite} to answer this query.
% %
% E.g., 

Parallel research has emphasized the use of \emph{contrastive reasoning} to assess causal explanations~\citep{cheng1991causes, hilton1990conversational, hilton1986knowledge, mcgill1989context, mackie1974cement}. In this line of reasoning, people ``contrast the target episode (the individual that was denied the loan) with instances in which the event did not occur (e.g., other employees who succeeded). Distinctive features between the target episode and contrasting instances are \emph{possible} \hl{causal explanations}.''



As suggested by \citet{mcgill1993contrastive, miller2019explanation}, ``both counterfactual and contrastive reasoning may be broadly classified as counterfactual, in that each considers instances in which some characteristic of the event (cause or effect) has been negated.'' \hl{negated/changed... we want to minimize the change, either in the effect (contrastive explanation) or in the cause (consequential interventions).}
%
In counterfactual \hl{reasoning/explanations}, one seeks the effect of \emph{negating the cause}, whereas in contrastive \hl{reasoning/explanations}, one aims to understand which causes that would lead to \emph{negation of the effect}.



This form of causal explanation through contrastive reasoning has grounding in the philosophy of science and how humans best understand and desire explanations \citep{miller2019explanation}.
%
Specifically, social science and psychology literature argue that all `why'-questions are of the form ``Why P, not Q?'' \hl{cite from Robeer}.
%
Human often don't care about the entire causal history (and it's often difficult to automatically learn anyways). 
%
``One does not explain an event per se, but that one explains why the puzzling event occured in the target cases but not in some counterfactual contrast case \hl{cite Hilton}.''


This finding is also an opportunity for XAI, as it is often easier to automatically find contrastive instances (i.e., with negated effects, in this case individuals who were offered the loan) and provide an explanation in terms of feature vectors differences, than it is to accurately infer the causal history (itself a difficult problem \hl{cite causal discovery}) and provide explanations based on negated causes. 
%
As we shall see below, most existing works have satisfyingly provided contrastive explanations, but not counterfactual ones.


Importantly, both counterfactual and contrastive reasoning are required for a complete assessment of causation \citep{mcgill1993contrastive, hilton1990conversational},
%
This distinction aligns well with the two questions we pose for recourse, which can be rewritten as:

\begin{enumerate}
    \item Who should I become in order to receive the loan?
    \item How should I become the aforementioned profile?
\end{enumerate}

In layman's terms,  ``inform an individual where they need to get to, and how to get there'' \citep{karimi2020mintrecourse}. 
In this context, contrastive explanations (with emphasize on the negated effect) seem to sufficiently answer the first question, and counterfactual explanations (with their emphasis on interventions in their causal history), seem better suited to answer the second question.
%

\amir{conclude with definitions of contrastive explanation, consequential interventions, and counterfactual instance}

Relative to a fixed decision-making model, earlier works in XAI consider recourse as the ``distance of an individual from the decision boundary of a classifier'' \citep{gupta2019equalizing, venkatasubramanianphilosophical}.
%
Complementarily, recent work has argued for the need of taking causal relationships between features into consideration when curating a set of recourse \emph{actions} for the individual \citep{karimi2020mintrecourse, karimi2020caterecourse}.


Graph that we described with Waleed. \hl{Reasoning, explanation, instance}



\subsection{Recourse in causally dependent worlds}
\label{sec:formulation_world}
\zmessage{ how the world works may not be necessary for understanding contrastive explanations, but it is taking actions.}

In the previous section we discuss the differences between contrastive and counterfactual, as well as their intended use in answering separate recourse questions.
%
However, a majority of existing literature on recourse seem to conflate these terms, which has resulted in inconsistent use of terminology and at times, over-claiming of what type of recourse an algorithm can provide (i.e., which of the two questions the methods answers).
%
Below, we discuss how this situation has risen from lack of consideration for the world in which actions are to be performed.

First observed by \citep{barocas2020hidden, venkatasubramanianphilosophical} and subsequently formalized by \citet{karimi2020mintrecourse}, most w...

%
This work shows that examples commonly used in the literature confuse the answer to the first question as an answer of the second question, and argue that previous work mistake contrastive explanations for actionable recommendations that the user can perform in order to achieve recourse.
%
Their argument, which is critical to properly distinguish between these questions and satisfying answer them, relies on the observation that negating some causes may have intermediary effects on other variables, which in turn may undesirably affect the target variable.
%
In summary, in an independent world (where input features/causes are independent), contrastive explanations may suffice as an answer for both questions, however, in most realistic settings, this assumption does not hold and thus, a different approach must be undertaken.

Thus
%
\emph{(nearest) counterfactual explanations} \citep{wachter2017counterfactual} and
\emph{(minimal) consequential interventions} \citep{karimi2020mintrecourse} 
%
have come into the limelight as approaches for answering both of the aforementioned questions, and thus endowing individuals with \hl{complete algorithmic recourse}.



In this work, we perform a broad survey of algorithmic recourse methods, and summarize the findings in \hl{Table ..} where we clearly demark the questions that each method satisfies.
%
In this regard, we note that generating meaningful recourse explanations/recommendations depends on additional factors such as similarity of causal history, minimality of effort, plausibility of counterfactuals, and feasibility of actions.
%
Although \emph{counterfactual explanations} -- ``how the world would have (had) to be different for a desirable outcome to occur'' -- and \emph{consequential interventions} -- ``a recommendable set of actions that would result in a counterfactual instance with a favourable output when performed'' -- are intuitively easy to understand \citep{wachter2017counterfactual, miller2019explanation}, generating such explanations/recommendations in diverse settings with desirable properties remains an open challenge.
%
Specifically, it is desirable to have one approach for generating explanations/recommendations for various objective measures, model classes, over real-world mixed-value datasets, and subject to various context-/individual-dependent plausibility and feasibility constraints.
%
Furthermore, the ideal generation method would identify explanations/recommendations for every individual in the population, efficiently (i.e., speedily), and at (near-)minimal distance/cost, across the settings above.
%
We explore these criteria in detail in the next sections.


\hl{see page 21 of wachter paper}

\hl{read ana lucic paper for good background mc-brp}

\hl{beyond separating explanations/recommendations, we shall see the implications of the world structure in the following section whereby the objective (\dist\, and \cost), as well as feasibility and plausibility definitions are teased apart accordingly}





==> _bu_020background_2021.01.19.tex <==

\subsection{Recourse definitions}
% \zmessage{recourse is guaranteed when two questions are answered.}
\amirm{3 def'ns}
In its relatively young field, algorithmic recourse has been defined as, e.g.,
``an actionable set of changes a person can undertake in order to improve their outcome'' \citep{joshi2019towards};
``the ability of a person to obtain a desired outcome from a fixed model'' \citep{ustun2019actionable};
or ``the systematic process of reversing unfavorable decisions by algorithms and bureaucracies across a range of counterfactual scenarios'' \citep{venkatasubramanianphilosophical}.
% It is argued that \hl{suresh things... temporally-extended agency and trust}
%
We submit that recourse can be achieved by an affected data-subject if they can \emph{understand} \citep{wachter2017counterfactual, joshi2019towards, downscruds} and accordingly \emph{act} \citep{karimi2020mintrecourse, karimi2020caterecourse} to alleviate an unfavorable situation, thus exercising temporally-extended agency \citep{venkatasubramanianphilosophical}.
%
\amirm{2 qqs}
Concretely, in the example of the previous section, recourse is offered when the loan applicant is given answers to both questions:
provided \emph{explanation(s)} as to why the loan was rejected (\textbf{Q1});
and offered \emph{recommendation(s)} on how to obtain the loan in the future (\textbf{Q2}).
%
Below, we describe the often overlooked difference between these questions and the different set of assumptions and tools needed to sufficiently answer each in general settings.

% Below we briefly review and clarify terminology, and describe the different set of assumptions needed for providing recourse.
% situating our argument in rich philosophical literature.


% \subsection{Philosophical foundations of recourse}
% \subsection{Recourse through \hl{a causal lens}}
%\subsection{Recourse through \hl{a philosophy lens}}
\subsection{Recourse and causality}
\label{sec:causal_recourse}

% In order to answer the two questions for recourse, we first remark on the form of explanations and recommendations used broadly in XAI (which subsumes consequential decision-making that focuses primarily on the data-subjects).


\subsubsection{\textbf{Contrastive Explanations}}
\amirm{def'n}
% \st{To provide explanations, we must first dissect the explanandum.}.\bernhard{I would tone it down a bit, and simply remove this (kind of) sentence - this will not help getting favorable reviews.}
%
In an extensive survey of the social science literature, \citet{miller2019explanation} concluded that when people ask ``Why P?'' questions, they are typically asking ``Why P rather than Q?'', where Q is often implicit in the context \citep{hilton1990conversational}.
%
A response to such questions is commonly referred to as a \emph{contrastive explanation}, and is appealing for two reasons.
%
Firstly, contrastive \emph{questions} provide a `window' into the questioner's mental model, identifying what they had expected (i.e., Q, the contrast case), and thus, the \emph{explanation} can be better tuned towards the individual's uncertainty and gap in understanding \citep{miller2018contrastive}.
%
% Secondly, as will become evident below
Secondly, providing contrastive explanations may be ``simpler, more feasible, and cognitively less demanding" \citep{miller2018contrastive} than offering recommendations. % \st{to both questioner and explainer}'' \bernhard{simpler than what? Or is this a (meta-) contrastive explanation of what a contrastive explanation is? ;)}\amir{thank you (and isabel) for pointing this out. in reviewing the source, while not clear, it seems the author means that contrastive explanations are simpler relative to \emph{causal attribution}-based explanations, which also aim to explain the causal relations between variables. Perhaps a small fix (with a bit of extrapolation) would be: ``simpler, more feasible, and cognitively less demanding'' than providing recommendations.}
% from a practical perspective and as we shall see below
% are asked when an individual is surprised of an event (e.g., loan rejection), where the contrast case identifies what the individual expected and is thus



\subsubsection{\textbf{Consequential Recommendations}}
\amirm{def'n}
Providing an affected individual with recommendations amounts to suggesting a set of \emph{actions} that should be performed to achieve a favourable outcome in the future.
%inferred actions directly from
In this regard, several works have used contrastive explanations to directly infer actionable recommendations \cite{karimi2020model, ustun2019actionable, sharma2019certifai, wachter2017counterfactual}, however, \citet{karimi2020mintrecourse} show that contrastive explanations may result in infeasible or suboptimal actions in general settings.
%
Instead, they suggest that actions should be interpreted as \emph{interventions} in a causal model of world in which actions will take place~\citep{karimi2020mintrecourse}.
%
Modelled in this manner, e.g., using a structural causal model (SCM) \citep{pearl2000causality}, the down-stream effects of interventions on other variables in the model (e.g., descendants of the intervened-upon variables) can directly be accounted for when recommending actions \citep{barocas2020hidden}.
%
% \citet{karimi2020mintrecourse} suggest that actions can be interpreted as \emph{interventions} in a causal model of the inter-variable relations, e.g., in a structural causal model (SCM) \citep{pearl2000causality}.
%
% Interventions may be performed additively \citep{eberhardt2007interventions} or structurally \citep{pearl2016causal}, and may stochastically change the value of multiple variables conditioned on a variety of pre-/post-intervention feasibility conditions. % in an additive manner
%
% Irrespective of the \emph{form}, \emph{feasibility}, and \emph{scope} of interventions, actions as interventions may have down-stream effects on other variables in the model (e.g., descendants of the intervened-upon variables) which should be accounted for when recommending actions \citep{barocas2020hidden}.
%
Thus a recommended set of actions for recourse, in a world governed by a SCM, are referred to as \emph{consequential recommendations} \citep{karimi2020mintrecourse, karimi2020caterecourse}.



\subsubsection{\textbf{Clarifying terminology: contrastive, consequential, \\ and counterfactual}}
\label{sec:clarifying_terminology}

Now that we understand that recourse explanations are sought contrastively, and that recourse recommendations can be considered as interventions on variables modelled using an SCM, 
%we ask how such explanations/recommendations are generated?
% we can define 
% \emph{contrastive explanations} -- ``how the world would have (had) to be different for a desirable outcome to occur'' --
% %
% and \emph{consequential recommendations} -- ``a recommendable set of actions that would result in a counterfactual instance with a favourable output when performed''.
%
we can rewrite the two recourse questions as:
\amirm{rewrite 2 qqs}
\begin{enumerate}
    % \item[\textbf{Q1.}] Who should I become in order to receive the loan? % \footnote{What profile would have received the loan?}
    \item[\textbf{Q1.}] What profile would have led to receiving the loan?
    \item[\textbf{Q2.}] What actions would have led me to develop this profile? % the aforementioned
\end{enumerate}


In layman's terms, recourse is offered when we ``inform an individual where they need to get to, and how to get there'' \citep{karimi2020mintrecourse}. 
%
For instance, a diabetic patient may know that a lower blood pressure would reduce their risk of heart failure, but only a doctor with better understanding of the underlying processes could effectively suggest ``interventions that will move the patient out of an at-risk group''~\citep{wachter2017counterfactual}.
%
\amirm{intuitively}
Viewed in this manner, both contrastive explanations and consequential recommendations can be classified as a \emph{counterfactual}~\citep{mcgill1993contrastive}, in that each considers the alteration of an entity in the history of the event P, where P is the undesired model output.
%
Thus, responses to \textbf{Q1} (resp. \textbf{Q2}) may also be called \emph{counterfactual explanations} (resp. \emph{counterfactual recommendations}), meaning what could have been (resp. what could have been done) \citep{byrne2019counterfactuals}.


% negation/alteration % of the fixed model. %, i.e., loan rejection. %instances in which some characteristic of the event P has been negated.
%
% The often overlooked differentiator between these recourse types is whether this alteration is performed independently or consequentially.

% \footnotetext{Alternatively, one may define \emph{counterfactual explanations} (resp. \emph{counterfactual recommendations}), \hbox{meaning what could have been (resp. what could have been done) \citep{byrne2019counterfactuals}.}}

\input{025figure}



To better illustrate the difference between contrastive explanations and consequential recommendations, we refer to Figure \ref{fig:contrastive_vs_consequential}.
%
According to \citet[p. 217]{lewis1986causal}, ``to explain an event is to provide some information about its causal history''.
%
\citet[p. 256]{lipton1990contrastive} argues that in order to explain why P rather than Q, ``we must cite a causal difference between P and not-Q, consisting of a cause of P and the absence of a corresponding event in the history of not-Q''.
%
% In the recourse setting, P and Q can be considered as the fixed model's output, i.e., loan approval and rejection, respectively.
%
% Moreover
\amirr{causal history}
% In the XAI\bernhard{define - explainable AI?}
In the algorithmic recourse setting, because the model outputs are determined by its inputs (which temporally precede the prediction), the input features may be considered as the causes of the prediction.
%
The determining factor in whether one is providing contrastive explanations as opposed to consequential recommendations is thus the level at which the \emph{causal history} \citep{ruben2015explaining} is considered:
% Importantly, this definition 
% Following this, the explainer does not need to reason about or even know about all causes of the fact — only those relative to the contrast case \citet{miller2018contrastive}.
%
% Specifically, whereas generating the former does not require knowledge of the causal relations between variables, generating the latter does.
% while explanations usually only go as far back as the model inputs, accounting for the consequences of actions requires modeling as far back as the causal generative process of the inputs including its dependence upon available actions. \iv{I would rewrite this sentence in terms of "while providing explanations only require information on the relationship between the model inputs and predictions, recommendations require information on the causal relationships among inputs."}\amir{thank you isabel!}
while providing explanations only requires information on the relationship between the model inputs, $\{\zrv{X}_i\}_{i=1}^D$, and predictions, $\hat{\zrv{Y}}$, recommendations require information as far back as the causal relationships among inputs. % (captured, e.g., in an SCM or a causal graph, both of which are non-identifiable from observational data alone \citep{peters2017elements}
%
The reliance on fewer assumptions \citep{miller2019explanation, lipton1990contrastive} thus explains why generating recourse explanations is easier than generating recourse recommendations.

% (i.e., assumptions on the parametric form of the SCM needed to compute $\xSCF$, or knowledge of the causal graph, both of which are non-identifiable from observational data alone \citep{peters2017elements})

% \amirr{offering expl. easier than recomm.}
% Alternatively, one my consider that generating contrastive explanations relies only on the parametric form of a human-designed decision-making system (which is fully specified), while generating consequential recommendations requires accurate knowledge of the SCM or a causal graph as a model of the nature itself (both of which are non-identifiable from observational data alone \citep{peters2017elements}).

% As we shall see in following section, generating contrastive explanations relies 
% fig 1 structural equations are the parametric form ebtween these relationships
% makign assumptipns on parametric form
% section 2historyt:
% right part is causal model, it is something we fix but doesn't exist in nature, we have the exact paramteric form (it's our mdel) known
% the left part is in the real worl we can make asumptions about but is not as easy to get
% features are measures of the world
% this is model this is real world



% usually only go as far back as the model inputs, accounting for the consequences of actions requires modeling as far back as the causal generative process of the inputs including its dependence upon available actions"}
% interventions model consequential actions based on the causal generative process.
%
% , however, ``counterfactuals generated from an accurate causal may ultimately be of use to experts'' \citep{wachter2017counterfactual}.
%
% \amirr{causality matters}
% To conclude this comparison, in an independent world (where input features are independent), contrastive explanations immediately yield (consequential) interventions resulting in recourse.
% %
% However, in most realistic settings, this assumption does not hold and thus, a different approach based on counterfactual inference is undertaken~\citep{karimi2020mintrecourse}.


% Importantly, offering recourse recommendations\bernhard{do you mean recommendations for actions?}\amir{indeed, i have tried to consistently use ``recourse/consequential recommmendations'' = ``actions'' (if in SCM framework=) ``interventions''.} implicitly provides recourse explanations as well (through simulation of the effect of the interventions), but the converse does not hold in general \citep{karimi2020mintrecourse}.\footnote{When input features are independent, interventions on one variable do not affect any other variable. Here, contrastive explanations immediately yield (non-consequential) interventions for recourse. However, this fails to hold in most real-world settings.}
% %
% In Table \ref{table:technical_summary}, we summarize the technical literature and specify the recourse questions that each paper answers (\textbf{Q1}: explanations \ee, or \textbf{Q2}: recommendations \rr).
% %
% As we shall see, most of the papers in the literature focus on offering explanations, primarily because of the additional assumptions needed to offer recommendations.


% the requirements above for explanations and recommendations align well with what is available in our setting, a fixed model, input variables, which for the purpose of contrastive explanation may be considered independent (minimum change in causal past, relative to the fixed model), but for recommendations, cannot be considered as such.


\amirm{generally hard}
% In this work, we perform a survey of algorithmic recourse, and summarize the technical literature in Table \ref{table:technical_summary}, specifying the recourse questions that each paper answers (\textbf{Q1}: explanations, or \textbf{Q2}: recommendations).
In Table \ref{table:technical_summary}, we summarize the technical literature and specify the recourse questions that each paper answers (\textbf{Q1}: explanations, or \textbf{Q2}: recommendations).
%
% As we shall see, by construction and through simulation of the causal history, consequential recommendations yield contrastive explanations, but not vice-versa.
% %
% As a result,
As we shall see, most of the literature focuses on offering explanations, primarily because of the additional assumptions needed to offer recommendations.
%
Furthermore, offering recourse in diverse settings with desirable properties remains an open challenge, which we explore in the following sections.
%
% Although contrastive explanations and consequential recommendations are intuitively easy to understand \citep{wachter2017counterfactual, miller2019explanation}, offering recourse in diverse settings with desirable properties remains an open challenge. % \hl{generating} recourse explanations/recommendations
%
% \hl{Such a task depends on factors such as similarity of causal history, minimality of effort, plausibility of counterfactuals, and feasibility of actions.}
%
% We explore these details in the following sections.
%
% Specifically, it is desirable to have one approach for generating explanations/recommendations for various objective measures, model classes, over real-world mixed-value datasets, and subject to various context-/individual-dependent plausibility and feasibility constraints.
% %
% Furthermore, the ideal generation method would identify explanations/recommendations for every individual in the population, efficiently (i.e., speedily), and at (near-)minimal distance/cost, across the settings above.
%
% We explore these criteria in detail in the next sections.


% % \hl{see p. 21 of wachter;}
% % \hl{read background in mc-brp paper}
% % \url{https://plato.stanford.edu/entries/causation-mani/}
% \amir{TODO: comment on interventionist theories to causality; on scientific vs everyday expl., \& something from Woodward}



==> _bu_050discussion.tex <==
\subsection{Related literature on CFE}

In the previous sections we covered the formulations and solutions of existing works aiming to offer recourse. While already quite general, there are a number of assumptions made in existing setups.

\hl{for benefits see p.22 of wachter}
\begin{itemize}
    \item \href{https://arxiv.org/pdf/1706.07269.pdf}{explanation in AI: insights from the social sciences}
    \item \href{https://www.semanticscholar.org/paper/The-philosophical-basis-of-algorithmic-recourse-Venkatasubramanian-Alfano/4627d3fd86423fe911ee40b8eb35b1e389ab41fd}{the philosophical basis of algorithmic recourse}
    \item \href{https://arxiv.org/pdf/1912.04930.pdf}{the hidden assumptions behind CFE and principle reasons}
    \item ``Promise''of CFE in \href{https://arxiv.org/pdf/2005.13997.pdf}{Good
    Counterfactuals and Where to Find Them}
    \item ``Perils'' of CFE in \href{https://www.nature.com/articles/s42256-019-0048-x}{stop explaining black-box ML models}
    \item why CFE are great explanations: \href{https://arxiv.org/abs/2005.01831}{Evaluating Explainable AI: Which Algorithmic Explanations Help Users Predict Model Behavior?}
\end{itemize}

also cite Kacper Sokol papers + \hl{Connectedness???????}

\subsection{Related literature elsewhere}
\begin{itemize}
    \item situate in grander context of XAI, and cite some of the review papers there
    \item mention relevance/importance of XAI in ascertaining other desiderata such as fairness
    \begin{itemize}
        \item \href{https://arxiv.org/pdf/1909.03166v1.pdf}{Equalizing Recourse across Groups}
        \item others i shared with Floyd
    \end{itemize}
    \item other desiderata, e.g., \href{https://arxiv.org/pdf/2006.12822.pdf}{Counterfactual Explanations of Concept Drift}
    \item relation to adversarial perturbations
    \item relation to inverse classification (and others in Ustun's work)
    \item \href{https://arxiv.org/pdf/2006.13132.pdf}{is the best classifier fixed?}
    \item machine teaching? 
\end{itemize}


\subsection{Limitations} % Dangers, and hazards
\begin{itemize}
    \item model stealing (even under only query access --> LUPI)
    \item misinterpretation of explanations as actionable recommendations
    \item lack of causal knowledge and thus lack of guarantee
    \item solutions requiring access to the training data, or to the model params
\end{itemize}


\subsection{Future directions}
\begin{itemize}
    \item other properties (e.g., path-connectedness suggested by Thibault Laugel, FACE, and program/conditional interventions)
    \item other properties (\href{https://www.ijcai.org/Proceedings/2019/0876.pdf}{Counterfactuals in XAI: Evidence from Human Reasoning})
    \item model-based approaches (rather than solving recourse for each individual independently)
    \item lack of benchmarks (formulations, datasets, and universal metrics), DUE TO user-/context-specific objective/cost, feasibility, etc.
    \item CFE focus primarily on the data-subject, but how about other stakeholders?
\end{itemize}


Finally, existing literature commonly assumes that a \emph{single} \emph{fixed} model is used to make decisions, and that recourse explanations/recommendations should be generated with respect to this model.
%
This assumption carries with it some subtle limitations that have been recently investigated in \cite{tsirtsis2020decisions, pawelczyk2020counterfactual, barocas2020hidden}. We summarize these discussions in \S~\hl{?}.


\subsection{From deterministic to probabilistic recourse}
In \eqref{eq:recommendation}, we saw that recourse actions could be obtained when the counterfactual instance, $\xCF$, is modelled as the structural counterfactual of $\xF$ under hypothetical actions $\actionVector$, i.e., $\xCF = \xSCF(\actionVector; \xF)$ \cite{karimi2020mintrecourse}.
%
Computing the structural counterfactual exactly, however, relies on strong assumptions (knowledge of the true structural causal model, and that the SCM is an additive noise model) that are often impractical in practical settings.
%
In fact, \citet{karimi2020caterecourse} show that without complete knowledge of the true SCM, counterfactual analysis cannot be done exactly and thus recourse cannot be deterministically guaranteed. These authors
%
While \citet{karimi2020caterecourse} then demonstrate how to probabilistically offer recourse with high probability, they do so under the assumption of knowledge of a causal graph without hidden confounding.
%
Future research in this direction may explore looser settings, perhaps with hidden confounding, or when the graph is partially observed.

Alternatively, sources of stochasticity may enter the explanation process via a non-deterministic decision-making system, such as those used in resource-limited settings. Consider a social service setting (e.g., housing for the homeless, tax audits), whereby the output of the model is a score/rank for the individual, after which the user is assigned a resource if they are randomly chosen according to their score amongst a pool of applicants.

\subsection{Beyond classification}
In \S\ref{sec:model} we discussed how the standard binary classification setting can be extended to support multi-class classification and regression.
%
Beyond these classic supervised learning settings, an individual may be subject to a (semi-)automated decision maker that determines a matching of applicants to resources across a population. E.g., kindergarten assignment for children, public housing for low-income families.
%
\hl{...}


\subsection{On the cost of recourse}
\label{sec:cost_of_recourse}
To capture the preference for actions with minimal cost/effort, or for small distance/dissimilarity between factual and counterfactual instances, existing approaches posit that distance/cost functions should satisfy the following properties:

\textbf{P1:} no action $\Leftrightarrow$ no cost $\Leftrightarrow$ no distance
\newline i.e., $\cost(\zvec{0}; \xF) = 0 = \dist(\xF, \xF)$ for $\xCFEnearest = \xF + \actionVectorStar$,
\newline and $\cost(\mathbbm{1}; \xF) = 0 = \dist(\xF, \xF)$ for $\xCFEnearest = \actionVectorStar \cdot \xF$

% \newline
\textbf{P2:} larger actions $\Leftrightarrow$ higher cost $\Leftrightarrow$ larger distance
\newline i.e., $\cost(\actionVector; \xF) \le \cost(\actionVector + \epsilon \mathbbm{1}_j ; \xF)$

While \textbf{P1} holds in both independent and dependent worlds, \textbf{P2} fails in dependent worlds where the cost of non-altering interventions -- necessary to ensure that $\xSCF$ equals $\xCFEnearest$ -- is overlooked.
%
For instance, the agriculture team in Example \#2 of \S\ref{sec:010introduction} may need to invest heavily in a greenhouse to ensure temperature remains the same if the paddy were to be situated at a different altitude.
%
A natural way to address this shortcoming is to distinguish between \emph{cost of actions} and \emph{cost of consequences of actions}, \hbox{equating the latter to the} cost of non-altering interventions.
%
This assignment holds intuitively: when consequences of actions are beneficial (detrimental) towards the output of $\htheta$, \hbox{the latter cost captures} the opportunity (preventative) cost of non-altering interventions.

The implementation of the proposed two-part cost function, however, involves a functional of not only $\actionVector$ and $\xF$, but also of $\scmModel$ and $\htheta$.
%
Furthermore, notions of cost and distance are notoriously difficult to design and not universally agreed upon \cite{dwork2012fairness, ilvento2019metric, venkatasubramanianphilosophical}.
%
In the spirit of not complicating matters further, we adopt the existing properties of cost functions (i.e., \textbf{P1}, \textbf{P2}), and propose a modification of \hl{eqn:nearest-cf-additive} that allows for \hl{actionSetStar} to \emph{optimally} and \emph{feasibly} follow via Option \#1, thereby avoiding the concerns of non-altering interventions.
%
% We present our approach in the following section, and defer the exploration of alternative cost definitions to future work.
\hl{talk also about cost of actions performed by fiduciary or background variables}.

\subsection{historical shaping of algorithmic phenomena; algorithmic impacts on social phenomena}

\hl{from FAccT CFP} \url{https://facctconference.org/2021/cfp.html}




% \subsubsection{\textbf{Beyond Optimization-based recourse}}
% model-based approaches (rather than solving recourse for each individual independently)







% \subsubsection{\textbf{New constraints / questions / defns for recourse?}}



% \subsubsection{\textbf{Recourse, gaming, and strategic classification}}
% \begin{itemize}
%     \item \url{https://arxiv.org/pdf/1910.10362.pdf} and others
%     \item \url{https://arxiv.org/pdf/2002.10066.pdf} agency is at odds with recourse?
%     \item \url{https://arxiv.org/pdf/2006.11638.pdf} influencing behavior change in population
%     \item \url{https://arxiv.org/abs/2002.04333}
%     \item \url{https://arxiv.org/abs/1910.05664}
% \end{itemize}

% \amir{also read page 4 of suresh paper}

==> _bu_060conclusions.tex <==
% \amir{TODO: rewrite}

\hl{Our work started with a case study of a 28-year-old female professional who was denied a loan by an automated decision-making system.}
%
In \S\ref{sec:010introduction}, we introduced \emph{algorithmic recourse} for this individual which was contingent on providing answers to two questions: why, and how?
%
In \S\ref{sec:020background}, we briefly reviewed relevant psychological and philosophical literature to shed light on the often overlooked causal differences underpinning these questions and argue that together, \emph{contrastive explanations} and \emph{consequential recommendations} satisfyingly offer recourse.
%
In \S\ref{sec:030formulation}, we formulate the tasks of recourse generation as constrained optimization problems with the objective of finding \emph{nearest} contrastive explanations \eqref{eq:explanation} and \emph{minimal} consequential recommendations \eqref{eq:recommendation}, and emphasize the latter to reduce the effort for the individual to achieve recourse. Here, additional real-world constraints covering actionability, plausibility, diversity, sparsity, and heterogeneous datatypes were also presented.
%
In \S\ref{sec:040solution}, we
% remark that the solving the optimization problems above are NP-hard, and
provide an overview of attempted solutions in the literature that trade-off between desirable properties such as optimality, efficient runtime, perfect coverage, and access.
%
Finally, in \S\ref{sec:050discussion}, we present a summary of the \emph{promises} and \emph{problems} of existing recourse approaches, and present \emph{prospects} towards which the community may engage, making explicit connections to other ethical challenges such as security, privacy, robustness, and fairness.
%
% Specifically, we pose and present potential solutions to the following questions:
% Specifically, we ask:

% \begin{enumerate}
%     \itemsep0em 
%     % \item[\textbf{Q2.}] How robust are recourse explanations/recommendations to changes in the model?
%     \item[\textbf{Q3.}] Does equalizing recourse across groups also satisfy other notions of fairness?
%     \item[\textbf{Q4.}] Does providing recourse for one individual violate the privacy of other individuals?
%     \item[\textbf{Q5.}] What information about the underlying model are we revealing when providing recourse?
%     \item[\textbf{Q6.}] Can an adversary use this revealed information to strategically game or manipulate the model?
%     % \item[\textbf{Q5.}] Does providing recourse explanations/recommendations put my model security at risk?
%     % \item[\textbf{Q5.}] How many recourse explanations/recommendations can I provide before risking model security?
% \end{enumerate}

Addressing such questions relies on the cross-disciplinary expertise of a panel of technical and social scientists.

To conclude, algorithmic recourse is the study of trade-offs:
% accuracy vs. explainability~\cite{gunning2019darpa, rudin2018please},
plausibility vs. coverage, %~\cite{karimi2020model},
assumptions vs. guarantees, %~\cite{karimi2020mintrecourse, karimi2020caterecourse},
efficiency vs. access, %~\cite{karimi2020sok},
optimality vs. collusion, %~\cite{milli2019model},
etc.
%
Beyond fostering trust with affected individuals, overcoming the opacity \cite{burrell2016machine} of such models is increasingly becoming a legal necessity for developers and deployers of said models \cite{wachter2017counterfactual, hsia1978credit} and in determining their adoption and impact \citep{fjeld2020principled}.
%
We hope that the presented document may guide further discussion and progress in this direction.

% \subsection{other..}
% Interpretability in ML is the study of \emph{trade-offs}: accuracy vs. explainability~\cite{gunning2019darpa, rudin2018please}, plausibility vs. coverage~\cite{karimi2020model}, optimality vs. collusion~\cite{milli2019model}, etc.


%     in this setting, we assume the model is given and we do post-hoc explanation. thus accuracy of underlying model is unaffected

% however, there is a tradeoff between the desired properties of recourse, such as sparsity, diversity, minimality/cost, etc.

% \amir{From AReS paper tradeoff between interp and recourse accuracy..; See bottom of page 3 of explaining explanations in ai}



